An Information Theoretic Perspective on Conformal Prediction

Conformal Prediction (CP) is a distribution-free uncertainty estimation framework that constructs prediction sets guaranteed to contain the true answer with a user-specified probability. Intuitively, the size of the prediction set encodes a general notion of uncertainty, with larger sets associated with higher degrees of uncertainty. In this work, we leverage information theory to connect conformal prediction to other notions of uncertainty. More precisely, we prove three different ways to upper bound the intrinsic uncertainty, as described by the conditional entropy of the target variable given the inputs, by combining CP with information theoretical inequalities. Moreover, we demonstrate two direct and useful applications of such connection between conformal prediction and information theory: (i) more principled and effective conformal training objectives that generalize previous approaches and enable end-to-end training of machine learning models from scratch, and (ii) a natural mechanism to incorporate side information into conformal prediction. We empirically validate both applications in centralized and federated learning settings, showing our theoretical results translate to lower inefficiency (average prediction set size) for popular CP methods.

==> tables/federated.tex <==
\begin{table*}[!t]
\centering
\caption{Inefficiency of conformal prediction in the federated setting with THR and APS for each dataset and for a target $\alpha = 0.01$. We report mean and standard deviation of the inefficiency of the global federated model, with and without side information, across 10 different calib./test splits and show in bold all values within one standard deviation of the best result. Lower is better.}
\label{tab:fed_results}
\resizebox{\textwidth}{!}{  
\begin{tabular}{ l@{\hskip 6pt} | c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 6pt} | c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 6pt} | c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 6pt} }
\toprule
 Method & \multicolumn{4}{c}{EMNIST} & \multicolumn{4}{c}{CIFAR 10} & \multicolumn{4}{c}{CIFAR 100} \\\midrule
 & THR & THR$_{+\text{side}}$ & APS & APS$_{+\text{side}}$ & THR & THR$_{+\text{side}}$ & APS & APS$_{+\text{side}}$ & THR & THR$_{+\text{side}}$ & APS & APS$_{+\text{side}}$ \\\midrule
CE & $2.91_{\pm 0.02}$  & $2.46_{\pm 0.02}$ & $3.69_{\pm 0.03}$ & $3.14_{\pm 0.04}$ & $2.73_{\pm 0.04}$  & $2.30_{\pm 0.06}$ & $\mathbf{2.83_{\pm 0.07}}$  & $2.43_{\pm 0.06}$ & $55.41_{\pm 1.09}$  & $52.31_{\pm 1.03}$ & $64.73_{\pm 0.34}$  & $62.67_{\pm 3.68}$  \\
\midrule
ConfTr & $4.60_{\pm 0.05}$  & $3.30_{\pm 0.02}$  & $6.14_{\pm 0.04}$  & $5.25_{\pm 0.04}$ & $10.00_{\pm 0.00}$  & $10.00_{\pm 0.00}$ & $10.00_{\pm 0.00}$  & $10.00_{\pm 0.00}$ & $\mathbf{45.60_{\pm 1.30}}$  & $\mathbf{41.18_{\pm 1.16}}$ & $55.18_{\pm 2.10}$  & $47.58_{\pm 1.48}$ \\
ConfTr$_{\text{class}}$ & $2.88_{\pm 0.02}$  & $\mathbf{1.98_{\pm 0.02}}$ & $\mathbf{2.65_{\pm 0.02}}$  & $\mathbf{2.42_{\pm 0.02}}$ & $3.53_{\pm 0.09}$  & $3.39_{\pm 0.08}$ & $10.00_{\pm 0.00}$  & $10.00_{\pm 0.00}$ & $58.53_{\pm 1.40}$  & $56.03_{\pm 1.29}$ & $99.92_{\pm 0.02}$  & $99.91_{\pm 0.01}$ \\
\midrule
Fano & $\mathbf{2.63_{\pm 0.02}}$  & $2.37_{\pm 0.02}$ & $3.12_{\pm 0.04}$  & $2.72_{\pm 0.03}$  & $\mathbf{2.39_{\pm 0.07}}$  & $\mathbf{2.07_{\pm 0.07}}$ & $\mathbf{2.73_{\pm 0.07}}$  & $\mathbf{2.39_{\pm 0.06}}$ & $\mathbf{47.91_{\pm 1.20}}$  & $\mathbf{41.19_{\pm 1.02}}$  & $\mathbf{46.95_{\pm 0.67}}$  & $\mathbf{42.75_{\pm 0.91}}$\\
MB Fano & $2.84_{\pm 0.04}$  & $2.25_{\pm 0.03}$ & $4.75_{\pm 0.03}$  &  $\mathbf{2.43_{\pm 0.01}}$ & $\mathbf{2.52_{\pm 0.07}}$  & $\mathbf{2.04_{\pm 0.07}}$ & $\mathbf{2.79_{\pm 0.13}}$  & $\mathbf{2.33_{\pm 0.05}}$ & $52.94_{\pm 1.40}$  & $46.97_{\pm 1.30}$ & $50.72_{\pm 1.77}$  & $45.72_{\pm 1.38}$ \\
DPI & $\mathbf{2.60_{\pm 0.02}}$  & $2.23_{\pm 0.01}$ & $2.98_{\pm 0.03}$  & $2.58_{\pm 0.02}$ & $2.76_{\pm 0.07}$  & $2.28_{\pm 0.03}$ & $\mathbf{2.68_{\pm 0.15}}$  & $\mathbf{2.22_{\pm 0.09}}$  & $52.36_{\pm 0.95}$  & $48.64_{\pm 0.70}$  & $51.29_{\pm 1.07}$  & $47.18_{\pm 1.27}$ \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/federated_noconf.tex <==
\begin{table*}[!t]
\fontsize{9pt}{9pt}\selectfont
\centering
\caption{Average prediction set size in the federated setting with THR and APS for each dataset and for a target $\alpha = 0.01$. We report mean and standard deviation of the inefficiency of the global federated model, with and without side information, across 10 different calib./test splits and show in bold all values within one standard deviation of the best result. Lower is better.}
\label{tab:fed_results}
% \resizebox{\textwidth}{!}{  
\begin{tabular}{ l@{\hskip 8pt}  c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 8pt}  c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 8pt}  c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 8pt} }
\toprule
 Method & \multicolumn{4}{c}{EMNIST} & \multicolumn{4}{c}{CIFAR 10} & \multicolumn{4}{c}{CIFAR 100} \\\midrule
 & THR & THR$_{\text{si}}$ & APS & APS$_{\text{si}}$ & THR & THR$_{\text{si}}$ & APS & APS$_{\text{si}}$ & THR & THR$_{\text{si}}$ & APS & APS$_{\text{si}}$ \\\midrule
CE & $2.91$  & $2.46$ & $3.69$ & $3.14$ & $2.73$  & $2.30$ & $\mathbf{2.83}$  & $2.43$ & $55.41$  & $52.31$ & $64.73$  & $62.67$  \\
\midrule
ConfTr & $4.60$  & $3.30$  & $6.14$  & $5.25$ & $10.00$  & $10.00$ & $10.00$  & $10.00$ & $\mathbf{45.60}$  & $\mathbf{41.18}$ & $55.18$  & $47.58$ \\
ConfTr$_{\text{class}}$ & $2.88$  & $\mathbf{1.98}$ & $\mathbf{2.65}$  & $\mathbf{2.42}$ & $3.53$  & $3.39$ & $10.00$  & $10.00$ & $58.53$  & $56.03$ & $99.92$  & $99.91$ \\
\midrule
Fano & $\mathbf{2.63}$  & $2.37$ & $3.12$  & $2.72$  & $\mathbf{2.39}$  & $\mathbf{2.07}$ & $\mathbf{2.73}$  & $\mathbf{2.39}$ & $\mathbf{47.91}$  & $\mathbf{41.19}$  & $\mathbf{46.95}$  & $\mathbf{42.75}$\\
MB Fano & $2.84$  & $2.25$ & $4.75$  &  $\mathbf{2.43}$ & $\mathbf{2.52}$  & $\mathbf{2.04}$ & $\mathbf{2.79}$  & $\mathbf{2.33}$ & $52.94$  & $46.97$ & $50.72$  & $45.72$ \\
DPI & $\mathbf{2.60}$  & $2.23$ & $2.98$  & $2.58$ & $2.76$  & $2.28$ & $\mathbf{2.68}$  & $\mathbf{2.22}$  & $52.36$  & $48.64$  & $51.29$  & $47.18$ \\
\bottomrule
\end{tabular}
% }
\end{table*}
